Piecewise-Linear Motion Planning amidst Static, Moving, or Morphing Obstacles

We propose a novel method for planning shortest length piecewise-linear motions through complex environments punctured with static, moving, or even morphing obstacles. Using a moment optimization approach, we formulate a hierarchy of semidefinite programs that yield increasingly refined lower bounds converging monotonically to the optimal path length. For computational tractability, our global moment optimization approach motivates an iterative motion planner that outperforms competing sampling-based and nonlinear optimization baselines. Our method natively handles continuous time constraints without any need for time discretization, and has the potential to scale better with dimensions compared to popular sampling-based methods.

==> Imgs/comparison_sos_rrt_nlp.tex <==
\begin{figure*}[htbp]
  \hspace{-1cm}
  \includegraphics[width=1.1\linewidth]{Imgs/comparison_sos_rrt_nlp}
  \caption{\label{fig:comparison_sos_rrt_nlp}SOS vs RRT vs NLP. In magenta, the smoothness. In blue, the length. (The shorter the better). We also report the running time}
\end{figure*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Path_Planning_Using_Moments"
%%% End:


==> Imgs/double_pendulum_experiment__Bachir_EL_KHADIR_s_conflicted_copy_2020-10-10_.tex <==
\begin{figure*}[htbp]
  \fbox{\includegraphics[width=\linewidth, trim= 5cm 5cm 2cm 2cm, clip]{Imgs/double_pendulum/double_pendulum_0.0.png}}
\end{figure*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Path_Planning_Using_Moments"
%%% End:


==> Imgs/setup_3d_moving_obstacles.tex <==

\begin{figure}
  \centering
\hspace{-1cm}
\begin{minipage}{.3\textwidth}
\includegraphics[trim=120 0 0 0,clip,width=1.2\textwidth]{Imgs/setup_3d_moving_obstacles_2.png}
\end{minipage}%
~%
\begin{minipage}{.15\textwidth}
  % Dummy figure to get the legend
 \begin{tikzpicture}
    \begin{axis}[%
    hide axis,
    xmin=10,
    xmax=50,
    ymin=0,
    ymax=0.4,
    legend style={draw=white!15!black,legend cell align=left}
    ]
    \addlegendimage{ultra thick, blue}
    \addlegendentry{Heuristic};
    \addlegendimage{ultra thick, green}
    \addlegendentry{RRT};
    \addlegendimage{ultra thick, pink}
    \addlegendentry{NLP}
    \end{axis}
  \end{tikzpicture}
\end{minipage}

\caption{\label{fig:setup_3d_moving_obs}Typical paths obtained for a motion
  planning problem in 3D. The path is constrained to be in the black box and
  should avoid the moving obstacles. Each obstacle is a sphere that moves with
  constant velocity (depicted by a red arrow).}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Path_Planning_Using_Moments"
%%% End:


==> Imgs/smiley_face.tex <==
\begin{figure}
  \centering

  % smiley face
  \begin{tikzpicture}
    [point/.style={circle,fill=blue!100,thick,
      inner sep=0pt,minimum size=5pt}]
    %\helpergrid{5}{5}

    \coordinate (X1) at (0, 0);
    \coordinate (X2) at (-.75, .5);
    \coordinate (X3) at (.75, .5);
    \coordinate (X4) at (.0, -.75);

    % face
    \draw[fill, gray!100] (X1) ellipse (2cm and 2cm);
    % left eye
    \draw[fill, white] (X2) ellipse (.5cm and .5cm);
    % right eye
    \draw[fill, white] (X3) ellipse (.5cm and .5cm);
    % mouth
    \draw[fill, white] (X4) ellipse (1.5cm and .25cm);
  \end{tikzpicture}
    \caption{Example of obstacles represented by semi-algebraic
    sets. $\{x_1^2+x_2^2 - 16 \ge 0, (x_1-3)^2+(x_2-2)^2 - 4 \ge 0,
    (x_1+3)^2+(x_2-2)^2 - 4 \ge 0, x_1^2+(x_2+3)^2 - 1 \ge 0\}$. The complement of the obstacles (the region where trajectories are allowed to live) is colored in gray.}
\end{figure}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Path_Planning_Using_Moments"
%%% End:

